The Zeta-Function of a p-Adic Manifold, Dwork Theory for Physicists

In this article we review the observation, due originally to Dwork, that the zeta-function of an arithmetic variety, defined originally over the field with p elements, is a superdeterminant. We review this observation in the context of a one parameter family of quintic threefolds, and study the zeta-function as a function of the parameter \phi. Owing to cancellations, the superdeterminant of an infinite matrix reduces to the (ordinary) determinant of a finite matrix, U(\phi), corresponding to the action of the Frobenius map on certain cohomology groups. The parameter-dependence of U(\phi) is given by a relation U(\phi)=E^{-1}(\phi^p)U(0)E(\phi) with E(\phi) a Wronskian matrix formed from the periods of the manifold. The periods are defined by series that converge for $|\phi|_p < 1$. The values of \phi that are of interest are those for which \phi^p = \phi so, for nonzero \phi, we have |\vph|_p=1. We explain how the process of p-adic analytic continuation applies to this case. The matrix U(\phi) breaks up into submatrices of rank 4 and rank 2 and we are able from this perspective to explain some of the observations that have been made previously by numerical calculation.

==> allcrossreferfile.tex <==
Equation quintic
Equation Upert
Equation quintic
Equation formzeta
Equation Fdef
Equation Fdef
Equation Fseries
Figure coneK
Equation nustarsum
Equation nustarG
Equation nustarG
Equation nustartrace
Equation DworkZ
Equation altprod
Equation innerprod
Equation nicond
Equation tildeUone
Equation coho
Equation Drels
Equation Uphi
Equation Utilde
Equation Utilde
Equation Qleqn
Equation Qleqntwo
Equation Xveqn
Equation Xveqn
Equation Xveqn
Equation Uzerov

